Learning to Use Tools via Cooperative and Interactive Agents

Tool learning empowers large language models (LLMs) as agents to use external tools and extend their utility. Existing methods employ one single LLM-based agent to iteratively select and execute tools, thereafter incorporating execution results into the next action prediction. Despite their progress, these methods suffer from performance degradation when addressing practical tasks due to: (1) the pre-defined pipeline with restricted flexibility to calibrate incorrect actions, and (2) the struggle to adapt a general LLM-based agent to perform a variety of specialized actions. To mitigate these problems, we propose ConAgents, a Cooperative and interactive Agents framework, which coordinates three specialized agents for tool selection, tool execution, and action calibration separately. ConAgents introduces two communication protocols to enable the flexible cooperation of agents. To effectively generalize the ConAgents into open-source models, we also propose specialized action distillation, enhancing their ability to perform specialized actions in our framework. Our extensive experiments on three datasets show that the LLMs, when equipped with the ConAgents, outperform baselines with substantial improvement (i.e., up to 14% higher success rate).

==> table/list_prompt.tex <==
\onecolumn
\makebox[\linewidth]{\rule{\linewidth}{0.4pt}}
\textit{The prompt to enable the \first in our cooperative framework. We detail the system prompt and input prompt, respectively.}
\begin{lstlisting}[basicstyle=\small\ttfamily, breaklines=true, breakindent=0em, commentstyle=\color{red!50!green!50!blue!50}, frame=shadowbox, rulesepcolor=\color{red!20!green!20!blue!20},numbers=none,literate={`}{\textasciigrave}1]

==== System prompt ====
In this task, you are provided a series of real-world APIs. Please give a solution to plan which API to use step-by-step to solve the user's query. Specifically, you should solve a query with interleaving Thought, Action, Observation steps.
You should break down the user's query into several simple sub-task. And give your Thought and Action step-by-step, waiting for the Observation to continue to give the subsequent solution.

Starting blow, you have to output in the following format
User query: the query a User wants help with related to the API.
Thought 1: the first step of your plan for how to solve the query
Action 1: Select just one API from the provided API list and output its API name
Observation 1: the result of executing the first step of your plan
Thought 2: based on the API response, the second step of your plan for how to solve the query. 
Action 2: Select just one API from the provided API list and output its API name
Observation 2: the result of executing the second step of your plan
... (this Thought and Action step can be repeated N times)
Thought N: The task is solved and the answer is [PROVIDE YOUR ANSWER]!
Action N: Finish

{examples}

In your Thought, You are encouraged to specify what key information you want to obtain from the full results or the selected API. For example, you are encouraged to give a plan "Find the **movie id** of the Matrix" instead of "Find the movie Matrix".

==== Input task ====

Here are the details of the APIs you can use. You can ONLY use the above APIs!
{Candidate toolset}

User query: {query} 
\end{lstlisting}


\onecolumn
\makebox[\linewidth]{\rule{\linewidth}{0.4pt}}
\textit{The prompt to enable the \second in our cooperative framework. We detail the system prompt and input prompt, respectively.}
\begin{lstlisting}[basicstyle=\small\ttfamily, breaklines=true, breakindent=0em, commentstyle=\color{red!50!green!50!blue!50}, frame=shadowbox, rulesepcolor=\color{red!20!green!20!blue!20},numbers=none,literate={`}{\textasciigrave}1]
==== System prompt ====

In this task, you should write Python code to call the following API according to my instructions. Note that: you should always `print` the final answer.


==== Input prompt ====
Here is the documentation of the API
{tool documentation}

Any information, e.g., person id or movie id, you need to obtain it by calling appropriate APIs. DO NOT make up value by yourself!
Instruction: {instruction} 
Your output: ```python 
Your Python code 
```
\end{lstlisting}


\makebox[\linewidth]{\rule{0.98\linewidth}{0.4pt}}
\textit{The prompt to enable the \third in our cooperative framework. We detail the system prompt and input prompt, respectively.}
\begin{lstlisting}[basicstyle=\small\ttfamily, breaklines=true, breakindent=0em, commentstyle=\color{red!50!green!50!blue!50}, frame=shadowbox, rulesepcolor=\color{red!20!green!20!blue!20},numbers=none,literate={`}{\textasciigrave}1]
==== System prompt ====
Please review my solution and evaluate whether my solution is correct.

==== Input prompt ====
My solution contains the Planning, Code, and Execution results.
Planning: the specific plan for how to solve the query
Code: the Python code snippet which calls the APIs to solve the question
Code output: the result of executing the Python code

Here is the tool documentation. 
{tool documentation}

Now, please review my solution. Your review should contain the type of error (planning error and Code error) and a clear instruction on how to fix it. 
(1) Planning error: The planning is vague, and lacks required arguments to call a function or does not explicitly state what information to extract from the function's return value.
(2) Code error: The planning is correct and specific, but the code encounters Python runtime errors, e.g., KeyError or TypeError.

Starting below,  please first identify the error type of my solution and then provide a clear instruction on how to fix it. Here are some review examples: 
{examples} 

Here is my specific solution.  
{solution}
 
Please give your review. 
Error: 

\end{lstlisting}

